Complex Ontology Matching with Large Language Model Embeddings

Ontology, and more broadly, Knowledge Graph Matching is a challenging task in which expressiveness has not been fully addressed. Despite the increasing use of embeddings and language models for this task, approaches for generating expressive correspondences still do not take full advantage of these models, in particular, large language models (LLMs). This paper proposes to integrate LLMs into an approach for generating expressive correspondences based on alignment need and ABox-based relation discovery. The generation of correspondences is performed by matching similar surroundings of instance sub-graphs. The integration of LLMs results in different architectural modifications, including label similarity, sub-graph matching, and entity matching. The performance word embeddings, sentence embeddings, and LLM-based embeddings, was compared. The results demonstrate that integrating LLMs surpasses all other models, enhancing the baseline version of the approach with a 45\% increase in F-measure.

==> figs/Figure_approach.tex <==
\begin{figure*}[ht!]
    \centering
    \makebox[\textwidth][c]{
    \begin{tikzpicture}[->,>=stealth]
    \matrix[nodes={draw, thick, font=\footnotesize}, row sep=0.9cm,column sep=2.3cm, ampersand replacement=\&,matrix of nodes] (source) at (0,0) { %
    \node[draw] (cqa) {CQA}; \& \node[draw] (e1) {$e_s$};   \\
      \& \node[draw] (Ls) {$L_s$}; \\
        \& \node[draw] (is) {$ans_s$}; \\
    } ; %endmatrix
    \matrix[nodes={draw, thick, font=\footnotesize}, row sep=1cm,column sep=2.3cm, ampersand replacement=\&,matrix of nodes] (target) at (8,0) { %
    \node[draw] (e2) {$e_t$}; \& \node[draw] (best) {Best Formulae};   \\
    \node[draw] (Lt) {$L_t$};  \&  \node[draw] (triple) {Subgraph}; \\
    \node[draw] (it) {$ans_t$}; \&  \node[draw,text width=2.5cm, align = center] (triples) {Subgraphs};\\
    } ; %endmatrix
    
   \draw  ($(source.south east)+(0.01,-0.01)$) rectangle  ($(source.north west)+(-0.01,0.2)$);
   \draw  ($(target.south east)+(0.4,-0.01)$) rectangle  ($(target.north west)+(-0.4,0.9)$);
   \draw [dashed] ($(triple.south east)+(0.2,-0.2)$) rectangle  ($(Lt.north west)+(-0.2,0.3)$);
    \node (sl) at ($(source.north)+(0,0.5)$) {Source};
    \node (tl) at ($(target.north)+(0,1.2)$) {Target};
    \node (forall) at ($(Lt.east)!0.3!(triple.west) + (0,0.8)$) {For each subgraph \circled{6}\circled{7}};
    
    \node[draw] (corres) at ($(target.north west)!0.5!(source.north east) + (-0.3,1.4)$) {Complex correspondence};

  \path (cqa) 
    edge node [pos=0.5, above] {\circled{1} DL formula} (e1)
    edge [in=180, out=270] node [pos=0.7, above] {\circled{2} URI labels} (Ls)
    edge [in=180, out=270] node [pos=0.5, right] {\circled{3} Answers} (is)
    (is) edge [in=180, out=0] node [pos=0.4, above] {\circled{4} Match} (it)
    (it) edge [in=180, out=0] node [pos=0.5, above] {\circled{5} Subgraphs} (triples)
    (triples) edge node [pos=0.5, right] {composed of} (triple)
    (triple) edge node [pos=0.5, above] {\circled{6} Retrieve labels} (Lt)
    (Lt) edge [in=0, out=180, decorate, decoration=snake] node [pos=0.6, above] {\circled{7} Compare} (Ls)
    (forall) edge [in=270, out=0] node [pos=0.8, right] {\circled{8}} (best)
    (best) edge[loop above] node [pos=0.8,above] {\circled{9} Counter examples} (best)
    (best) edge node [pos=0.5, above,text width=2cm] {\circled{10} Filter} (e2)
    (e2) edge[in=290, out=180,] node [pos=0.8,right] {\circled{11} } (corres)
    (e1) edge[in=260, out=0,] node [pos=0.8,left] {\circled{11} } (corres) ; 
    \end{tikzpicture}
    }
    
    \caption{Schema of the general approach.}
    \label{fig:approach}
    \vspace{-0.2cm}
\end{figure*}

==> figs/cqa1.tex <==
\begin{minipage}{0.5\linewidth}
\begin{lstlisting}
SELECT ?x WHERE {
  ?x a o1:AcceptedPaper.
}
\end{lstlisting}
\end{minipage}


==> figs/cqa2.tex <==
\begin{minipage}{0.5\linewidth}
\begin{lstlisting}
SELECT ?x ?y WHERE {
  ?x o1:paperWrittenBy ?y.
}
\end{lstlisting}
\end{minipage}

==> figs/d1.tex <==
\begin{tikzpicture}[scale=0.8]
\footnotesize
		\tikzstyle{class}=[draw,rounded rectangle, color = blue, text = blue, minimum size = 0.7cm]
		\tikzstyle{inst}=[draw, rectangle]
	\node[class] (pap) at (0,3){\oun:Paper};
	\node[class] (acc) at (0,1.5){\oun:AcceptedPaper};
	
	\node[inst] (pap1) at (0,0){\oun:paper1};
	
	\node[class] (pers) at (-7,1.5){\oun:Person};
	\node[inst] (pers1) at (-7,0){\oun:person1};

	\path[->,draw,thick]
	(acc) edge[pil,right]node[prop]{rdfs:subClassOf}(pap)
	(pap1)edge[pil,left,in=180, out=180] node[prop] {rdf:type} (pap)
	(pap1)edge[pil,right] node[prop] {rdf:type} (acc)
	
	(pap1)edge[pil,above] node[prop] {\oun:paperWrittenBy} (pers1)
	(pers1)edge[pil,right] node[prop] {rdf:type} (pers);

	\end{tikzpicture}

==> figs/d2.tex <==
	\begin{tikzpicture}[scale=0.8]
\footnotesize
		\tikzstyle{class}=[draw,rounded rectangle, color = blue, text = blue, minimum size = 0.7cm]
		\tikzstyle{inst}=[draw, rectangle]
	\node[class] (dec) at (-6,-3){\odeux:Decision};
	\node[class] (acc) at (0,-3.){\odeux:Acceptance};
		
	\node[inst] (dec1) at (0,-1.5){\odeux:decision1};
	
	\node[inst] (pap1) at (0,0){\odeux:paper1};
	
	\node[class] (pap) at (0,1.5){\odeux:Paper};
	\node[class] (doc) at (0,3){\odeux:Document};
	\node[inst] (pers1) at (-5.5,0){\odeux:person1};
	\node[class] (pers) at (-5.5,1.5){\odeux:Person};

	\path[->,draw,thick]
	(acc) edge[pil,above]node[prop]{rdfs:subClassOf}(dec)
	(pap) edge[pil,right]node[prop]{rdfs:subClassOf}(doc)
	(dec1)edge[pil,left] node[prop] {rdf:type} (acc)
	(dec1)edge[pil,left,out=170] node[prop] {rdf:type} (dec)
	(pap1)edge[pil,left] node[prop] {\odeux:hasDecision} (dec1)
	(pap1)edge[pil,right] node[prop] {rdf:type} (pap)
	(pap1)edge[pil,left,out=170,in=180] node[prop] {rdf:type} (doc)
	(pers1)edge[pil,above] node[prop] {\odeux:writes} (pap1)
	(pers1)edge[pil,left] node[prop] {rdf:type} (pers)
;

	\end{tikzpicture}
